Isolation and Impartial Aggregation: A Paradigm of Incremental Learning without Interference

This paper focuses on the prevalent performance imbalance in the stages of incremental learning. To avoid obvious stage learning bottlenecks, we propose a brand-new stage-isolation based incremental learning framework, which leverages a series of stage-isolated classifiers to perform the learning task of each stage without the interference of others. To be concrete, to aggregate multiple stage classifiers as a uniform one impartially, we first introduce a temperature-controlled energy metric for indicating the confidence score levels of the stage classifiers. We then propose an anchor-based energy self-normalization strategy to ensure the stage classifiers work at the same energy level. Finally, we design a voting-based inference augmentation strategy for robust inference. The proposed method is rehearsal free and can work for almost all continual learning scenarios. We evaluate the proposed method on four large benchmarks. Extensive results demonstrate the superiority of the proposed method in setting up new state-of-the-art overall performance. \emph{Code is available at} \url{https://github.com/iamwangyabin/ESN}.

==> 03_approach_back.tex <==
\section{Methods}

\subsection{Problem Definition}

Incremental learning is defined as training the model in data stream, and the model can only access part of training data at a time.
A data stream of $S$ sessions can be formulated as $\mathcal{D} =\left \{ \mathcal{D}_1, \mathcal{D}_2, ..., \mathcal{D}_S \right \} $.
The incoming data of $s$-th session is $\mathcal{D}_s = \left \{  x_i^s,y_i^s \right \}_{i=1}^{N_s}$, where $x_i^s$ is the $i$-th input image from session $s$ and $y_i^s$ is the corresponding label, and the total number of samples at session $s$ is ${N_s}$.
Total categories is $\mathcal C$. 
For class incremental learning, different session have different categories to learn, and there is no category overlap.
Thus categories can be formulated as $\mathcal{C} = \left \{ \mathcal{C}_1, \mathcal{C}_2, ..., \mathcal{C}_S \right \} $, where $\mathcal{C}_s$ is the categories need to be learnt on session $s$.
For domain incremental learning, the categories maintains the same for all sessions, but each session $s$ has data $\mathcal D_s$ from different or even highly heterogeneous domains .


\subsection{Overview.}

Traditional incremental learning methods tackle the catastrophic forgetting by designing regularization strategies and building rehearsal memory.
However, storing previous sessions' data requires a lot of storage space, and old knowledge will inevitably be forgotten.
In this paper, we focus on the exemplar-free incremental learning problem, which means the algorithm can not store any raw training data.
This is a more practical scenario for better data security, privacy and cheaper memory consumption.
To address the exemplar-free incremental learning problem, we propose an out-of-distribution incremental learning paradigm that is simple and effective. 
The key idea of out-of-distribution incremental learning is each network has enough ability to distinguish judge whether the test sample belongs to its session.
Thus the network can learn new knowledge session by session independently.

The key problem of our method is that we need completely independent networks for different sessions, and we can aggregate these networks by our OOD strategy.
The intuitive idea is to learn new network for every sessions like DER~\cite{}.
What's more, many existing parameter isolation incremental learning~\cite{} and finetuning~\cite{} methods can use our method to achieve incremental learning.
Designing a very appropriate parameter efficient tuning strategy in the field of incremental learning is not the focus of our research. 
This paper tries to aggregate independent networks for incremental learning.
Therefore, we use a simple baseline, that is, only adding a lightweight decoder layer to the backbone network to learn the current task.
Though this may cost more memory than using prompt method, but this can save much inference time.
We will show that using prompt tuning can also achieve our purpose. 

Given a pre-trained backbone $f_{\theta}$, every session we initialize a decoder $f_{\eta_s}^s$, a classifier $f_{\tau_s}^s$.
And $\theta$, $\eta$ and $\tau$ are parameters of backbone, decoder and classifier respectively.
During training, we freeze the pre-trained backbone $f_{\theta}$ and only update parameters of the decoder $\eta_s$ and classifier $\tau_s$.

The decoder layer is a lightweight Task-Attention Block~\cite{}, which is similar transformer self-attention block.
The output embedding of backbone is directly fed into the decoder layer, and the final output then fed to a classifier.
The classifier is a linear projection.

Different from the original multi-class out-of-distribution detection problem only has one classifier and using the confidence score (such as maximum SoftMax value~\cite{}, energy~\cite{}, entropy~\cite{}) and a single threshold to determine whether samples are belonging to the in-distribution or the out-of-distribution. Our method has multiple classifiers, and only need to select the most competitive classifier with the highest confidence score. The most challenging problem is to align the confidence scores between different classifiers. 


\subsection{Out-of-distribution based Incremental learning.}

The training process is completely independent and is almost the same as general classification tasks.
We use Cross-entropy to optimize session independent classification models, which is commonly used in machine learning.
Let $h^s(x)=f_{\tau_s}^s( f_{\eta_s}^s ( f_{\theta} (x))  )$ be the logits of the input sample image $x$ of session $s$ network. 
The softmax cross-entropy loss is as Eq.~\ref{eq:celoss}.
\begin{equation}
    \mathcal{L}_{ce} = -\sum_{c=1}^{C} y_c \log \frac{ \exp (h(x)_c) }{\sum_{i=1}^{C} \exp ( h(x)_i ) }.
\label{eq:celoss}
\end{equation}


In this paper, we show that using the simple out-of-distribution baseline method, Maximum softmax probabilities (MSP), can handle the incremental learning, including class-incremental learning and domain incremental learning.
MSP uses the maximum softmax probability as the confidence score, as Eq.~\ref{eq:msp}.
\begin{equation}
    Score_{\mathrm{MSP}}^s (x)= \max_{i=1,...,C_s}  \sigma _i ^s(x).
    \label{eq:msp}
\end{equation}
where $x$ is the input sample, and total categories is $k$, $\sigma _i ^s(x)$ is the probability of $x$ belong to category $i$ using $s$-th classifier as Eq.~\ref{eq:siga}.
\begin{equation}
    \sigma _i ^s (x)=\frac{\exp (h^s(x)_i)}{ {\textstyle \sum_{j=1}^{C_s} \exp(h^s(x)_j)} }.
    \label{eq:siga}
\end{equation}
Different from out-of-distribution detection scenario, and we do not set threshold to determine which session this image belongs to.
Instead we can use the maximum prediction over of all session as Eq.~\ref{eq:pred}.

\begin{equation}
    \hat{y} = \mathrm {argmax}_{s=1,...,S}(\sigma _i ^s)
    \label{eq:pred}
\end{equation}


However, the classifiers of different sessions would have biases, especially different session may have a large deviation.
Thus using multiple MSP scores for prediction has great uncertainty for incremental learning scenario.
The energy is defined to be the -logsumexp of logit outputs.
We propose a alignment loss based on energy theory as Eq.\ref{eq:energy_align}.
\begin{equation}
    \mathcal{L}_{energy} = \left \| -\log{\sum_{i=1}^{C_s} \exp (h^s(x)_i) }  - E_{anchor} \right \|  ^ 2.
\label{eq:energy_align}
\end{equation}
where $E_{anchor}$ is the anchor energy we set, which is $-10$ in implementation.
The total loss to training model on session $s$ as Eq.\ref{eq:total}.
\begin{equation}
    \mathcal{L} = \mathcal{L}_{ce} + \lambda  \mathcal{L}_{energy}.
\label{eq:total}
\end{equation}
where $\lambda$ is a parameter to balance $\mathcal{L}_{energy}$ term, which is $0.1$ in practice.
The proposed energy alignment strategy can correct the OOD bias of different classifiers.


\begin{figure}[H] 
\centering
\includegraphics[width=0.5\textwidth]{Figs/distcomp.pdf} 
\caption{Distribution shift.} 
\label{fig:distcomp} 
\end{figure}



\begin{algorithm}[t]
\begin{algorithmic}[1]
\item \textbf{Given components:} Pre-trained transformer-based backbone $f_{\theta}$, Total learnt sessions $S$, Training iterations for each session $M$, Anchor energy $E_{anchor}$, Training data $\mathcal{D}$, Learning rate $\epsilon$;
\FOR{$s = 1,\cdots,S$} 
  \item Initialization classifier $f_{\tau_s}^s$ and decoder $f_{\eta_s}^s$ for session $s$.
  \FOR {$m = 1,\cdots,M$}
    \item Draw a mini-batch training data $B=\left \{ x, y \right \} $ from $\mathcal{D}_s$
    \item Calculate prediction logits $h^s(x)=f_{\tau_s}^s( f_{\eta_s}^s ( f_{\theta} (x)))$
    \item Calculate loss $\mathcal{L}_B$ by Eq.\ref{eq:celoss}, Eq.\ref{eq:energy_align} and Eq.\ref{eq:total}
    \item Update $\tau_s$ by $\tau_s \gets \tau_s - \epsilon \bigtriangledown_{\tau_s} \mathcal{L}_B $
    \item Update $\eta_s$ by $\eta_s \gets \eta_s - \epsilon \bigtriangledown_{\eta_s} \mathcal{L}_B $
  \ENDFOR
  \item Saving $\tau_s$ and $\eta_s$.
\ENDFOR
\end{algorithmic}
\caption{Method at train time}
\label{alg:algo_train}
\end{algorithm}

\subsection{Temperature Calibration Voting Strategy}
As mentioned above, the key problem of applying OoD to incremental learning is how to deal with the predictions obtained by different detectors.
If all detector are trained equally well, the simplest way is Eq.~\ref{eq:pred}.
And we design the energy anchor loss to guide all detectors.
However, it is inevitable that there will be some inconsistency among classifiers.

Temperature scaling is a technique that divides the logits by a temperature (hyper)parameter and has been shown to improve OoD detection performance.
Larger temperature can yield more diffuse probability estimates.
For given detector, different detectors  may have different predictions.
If the detector perform consistency across various temperatures, it‘s result would be more reliable than detectors perform inconsistency.
For we align the energy of different learnt classifiers, we can use a uniform hard voting strategy to get the prediction.


The temperature-scaled softmax score for class $i$ is as Eq.~\ref{eq:tempsoftscore}.
\begin{equation}
    \label{eq:tempsoftscore}
    \sigma _i ^s \left ( x; t \right ) =\frac{\exp \left ( h^s(x)_i / t \right ) }{ {\textstyle \sum_{j=1}^{C} \exp \left ( h^s(x)_j / t \right )} }
\end{equation}

where the parameter $t$ is the temperature,

The prediction on temperature $t$ is as Eq.~\ref{eq:pred_T}.
\begin{equation}
    \hat{y}^t = \mathrm {argmax}_{s=1,...,S}(\sigma _i ^s (x;t))
    \label{eq:pred_T}
\end{equation}

we predict the class label $\hat{y}$  via majority (plurality) voting of each temperature as Eq.~\ref{eq:voting}.
\begin{equation}
    \hat{y} = mode\left \{ \hat{y}^1,...,\hat{y}^T \right \} 
    \label{eq:voting}
\end{equation}
where $T$ is the maximum temperature for voting.

The calculation cost of calculating the prediction results of different temperature can be neglected.
But this strategy can largely enhance the final prediction accuracy.

\begin{algorithm}[t]
\begin{algorithmic}[1]
\item \textbf{Given components:} Pre-trained transformer-based backbone $f_{\theta}$, trained classifiers $\{f_{\tau}^s\}_{s=1}^S$,  trained decoders $\{f_{\eta}^s\}_{s=1}^S$, Max temperature $T$, Total learnt sessions $S$ 
\item \textbf{Input:} test example $x$ 
\item Calculate image feature $l(x) = f_{\theta}(x)$ 
\FOR{$s = 1,\cdots,S$} 
  \item Generate $s$-th logits $h^s(x)=f_{\tau_s}^s( f_{\eta_s}^s (l(x)))$
  \FOR {$t = 1,\cdots,T$}
    \item Calculate temperature scaled softmax score $\sigma _i ^s \left ( x; t \right )$ by Eq.~\ref{eq:tempsoftscore}
  \ENDFOR
\ENDFOR
\item Get prediction on temperature $t$ by Eq.\ref{eq:pred_T}
\item Voting to get final prediction $\hat{y}$ by Eq.~\ref{eq:voting}

\end{algorithmic}
\caption{Method at test time}
\label{alg:algo_test}
\end{algorithm}

